A Model for Assessing Network Asset Vulnerability Using QPSO-LightGBM

With the continuous development of computer technology and network technology, the scale of the network continues to expand, the network space tends to be complex, and the application of computers and networks has been deeply into politics, the military, finance, electricity, and other important fields. When security events do not occur, the vulnerability assessment of these high-risk network assets can be actively carried out to prepare for rainy days, to effectively reduce the loss caused by security events. Therefore, this paper proposes a multi-classification prediction model of network asset vulnerability based on quantum particle swarm algorithm-Lightweight Gradient Elevator (QPSO-LightGBM). In this model, based on using the Synthetic minority oversampling technique (SMOTE) to balance the data, quantum particle swarm optimization (QPSO) was used for automatic parameter optimization, and LightGBM was used for modeling. Realize multi-classification prediction of network asset vulnerability. To verify the rationality of the model, the proposed model is compared with the model constructed by other algorithms. The results show that the proposed model is better in various predictive performance indexes.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Table/Algorithm1.tex <==
\begin{algorithm}[ht]
    \caption{Respiration Detection}
    \label{algorithm:breathDetect}
    \LinesNumbered
    \KwIn {$ L $  /* Sliding window size */    \\
           $ A $  /* Amplitude of CSI ratio samples after filtering */
        }
    \KwOut {$S_1$ /* Samples of PFT motions */}
    
    $ Vars[1:N] \leftarrow$ Variances on sliding windows of amplitude $\sum_{i=1}^{L}  (A_{i} - \overline{\mu})^2 $ \; 
    
    $ Peaks[1:K] \leftarrow $ Find peak indexes of $Vars[1:N]$ \; 
    
    \For{i $\leftarrow$ 1 to K} {
        $n \leftarrow Peaks(i)$ \;
        \If{ $Vars(n)$ $\geq$ threshold \textbf{and}  $\sum_{j=n}^{(n + L')}Vars(j) \geq \sum_{(j=n-L')}^{n}Vars(j) $ }{
            $ pStart \leftarrow $ Find the first valley to the left\; 
            break\;
        }
    }
    
    $ pEnd \leftarrow $ Similar to above but with contrast direction.
    
    $ S_1 \leftarrow R (pStart : pEnd)$
    
\end{algorithm}

==> Table/Algorithm2.tex <==

\begin{algorithm}[ht]
    \caption{Noisy Motion Remover}
    \label{algorithm:forwardMotion}
    \LinesNumbered
    \KwIn {$ S_1 $  /* Output of Algorithm 1 */
        }
    \KwOut {$ S_2 $ /* A clean inspiration-expiration process. */}
    
    $ Tan[1:N] \leftarrow $ Tangent between two adjacent samples: $ {(S_{1Q}(i+1) - S_{1I}(i))}/{(S_{1I}(i+1) - S_{1I}(i))} $ \; 
    
    $ R[1:N-1] \leftarrow $Rotation between two adjacent samples $ Tan(i) \times Tan(i + 1) $ \;
    
    $ CZ[1:K] \leftarrow $ Find cross zero indexes of rotation $R$  \;
    
    \If{$ CZ $ is not empty}{
        $ minR \leftarrow $ Minimum of rotation $R$ \;
        $ Valleys[1:M] \leftarrow $ Find valley indexes of $R$\;
        
        \For{$i \leftarrow$ 1 to M}{
            n $\leftarrow Valleys(i) $\;
            \If{$ R(n) \leq threshold * minR$}{
                $ pStart \leftarrow $ Find the first CZ to the left \;
                $ pEnd \leftarrow $ Find the first CZ to the right \;
                break\;
            }
        }
    }
    
    $ S_2 \leftarrow S_1 (pStart : pEnd)$
\end{algorithm}

==> Table/Algorithm3.tex <==

\begin{algorithm}[ht]
    \caption{Backward Motion Reduction}
    \label{algorithm:backwardMotion}
    \LinesNumbered
    \KwIn { $ L  $  /* Sliding window size */    \\
            $ W2 $  /* Output of Algorithm 2 */ }
    \KwOut {$ W3 $ /* Samples without small backward motion. */}
    
    % $ ruler1[N-L] = $ Amplitude variance with sliding window \;
    % $ ruler2[N-L] = $ Phase change of $ W2 $ with sliding window \;
    % $ ruler3[N-L] =  ruler2 ./ ruler1$ \;
    $ ruler1= $ Amplitude variance with sliding window \;
    $ ruler2 = $ Phase change of $ W2 $ with sliding window \;
    $ ruler3 =  ruler2 ./ ruler1$ \;
    
    $ I[1:K] = $ Find peaks indexed of $ ruler3 $ \;
    
    \For{i = 1 to K}{
        \If{ $ ruler3(I(i)) \leq $ thresh1 \textbf{and} $ruler1(I(i)) \geq $ 
        thresh2}{
            I(i) = null;  /* Remove unqualified peaks */ \;
        }
    }
    
    $ Sects[1:M] \leftarrow $ Find the interval indexes of peaks \;
    
    $ s[1:2] \leftarrow $ Find the interval with maximum of ruler1\;
    
    $W3 \leftarrow W2(s(1):s(2))$
\end{algorithm}

==> Table/Corr.tex <==
% \begin{table}[ht]
%     \caption{ Correlation between Human Factors and lung function indices ($\%pred$). }
%     \label{tab:correlation}
%     \centering
%     \begin{tabular}{|l|c|c|c|}
%         \hline
%         \textbf{Corr. Coeff.} & \textbf{FVC} & \textbf{FEV1} & \textbf{FEV1/FVC} \\
%          \textbf{(P-value)} & {} & {} & {}\\
%          \hline
%     Gender & 0.53(0.02) & 0.58(0.01) & 0.25(0.32)  \\
%     \hline

%     High Blood Pressure & 0.009(0.97) & 0.08(0.75) & 0.34(0.17) \\
%     \hline  

%     Coronary Heart & 0.09(0.72) & 0.13(0.60) & 0.25(0.32) \\
%     \hline  
    
%     Heart failure & 0.33(0.20) & 0.35(0.17) & 0.09(0.70)  \\
%     \hline
    
%     Brain Infarction & 0.08(0.75) & 0.09(0.73) & 0.003(0.99)\\
%     \hline   
    
%     \end{tabular}
%     %\caption{Caption}
    
% \end{table}

\begin{table}[ht]
    \caption{ Correlation between Human Factors and lung function indices. }
    \label{tab:correlation}
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        \textbf{Corr. Coeff.} & \multirow{2}{*}{\textbf{FVC}} & \multirow{2}{*}{\textbf{FEV1}} & \multirow{2}{*}{\textbf{FEV1/FVC}} \\
         \textbf{(P-value)} & {} & {} & {}\\
         \hline
    \multirow{2}{*}{Gender} & 0.53 & 0.58 & 0.25 \\
    {} & (0.02) & (0.01) & (0.32) \\
    \hline
    \multirow{2}{*}{Age} & 0.42 & 0.46 & 0.06 \\
    {} & (0.09) & (0.06) & (0.82)\\
    \hline

    \multirow{2}{*}{High Blood Pressure (HBP)} & 0.009 & 0.08 & 0.34 \\
    {} & (0.97) & (0.75) & (0.17) \\
    \hline  

    \multirow{2}{*}{Coronary Heart (CH)} & 0.09 & 0.13 & 0.25\\
    {} & (0.72) & (0.60) & (0.32)  \\
    \hline  
    
    \multirow{2}{*}{Heart Failure (HF)} & 0.33 & 0.35& 0.09  \\
    {} & (0.20) & (0.17)  & (0.70) \\
    \hline
    
    \multirow{2}{*}{Brain Infarction (BI)} & 0.08 & 0.09& 0.003\\
    {} & (0.75) & (0.73)  & (0.99) \\
    \hline   
    
    \end{tabular}
    %\caption{Caption}
    
\end{table}

==> Table/CorrLab.tex <==
\begin{table}[ht]
    \caption{ Correlation between Human Factors and lung function indices. }
    \label{tab:correlation:lab}
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        \textbf{Corr. Coeff.} & \multirow{2}{*}{\textbf{FVC}} & \multirow{2}{*}{\textbf{FEV1}} & \multirow{2}{*}{\textbf{FEV1/FVC}} \\
         \textbf{(P-value)} & ~ & ~ & ~\\
         \hline
    \multirow{2}{*}{Gender} & 0.90 & 0.83 & 0.31 \\
    ~ & (0.008) & (0.006) & (0.31) \\
    \hline

    \multirow{2}{*}{Age} & 0.31 & 0.35 & 0.16 \\
    ~ & (0.41) & (0.35) & (0.16) \\
    \hline  

    Body Mass  Index & 0.70 & 0.70 & 0.09\\
    (BMI) & (0.04) & (0.04) & (0.81)  \\
    \hline  
    
    \end{tabular}
    %\caption{Caption}
    
\end{table}

==> Table/Table1.tex <==
\begin{table*}[htbp]
\caption{Comparison of technologies measuring human breathe volume out of clinic}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{} & \textbf{Signal} & \textbf{Sensing} & \textbf{Physical} & \textbf{Specialized} & \textbf{Clinical} & \textbf{Performance}  \\
\textbf{} & \textbf{} & \textbf{range} &  \textbf{contact} & \textbf{device}  & \textbf{validation} & \textbf{} \\
\hline

Gupta, 2011\cite{Gupta11sensor} & Sensor  &  0m & Yes & Yes & Limited & Flow detection rate: $\geq 92\% $ \\
{} & {} & {} & {} & {} & {} & cough detection rate: $\geq 95\% $ \\
\hline

Chu, 2019 \cite{Chu19sensor} & Sensor & 0m & Yes & Yes & Limited & Correlation coefficient: $0.929 \sim 0.962$ \\
\hline

Lewis, 2011 \cite{Lewis11vision} & Vision & & No & Yes & None &  Within-Subject correlation: $0.9$\\
\hline

Yu, 2012 \cite{Yu12vision} & Vision &   & Yes & Yes & None & Correlation coefficient: $r=0.966$\\
\hline

Larson, 2012 \cite{Larson12Spirosmart} & Sound & & No & No & Limited & Compared to a clinical spirometer: $ 5.1\% $ \\
\hline

Goel, 2016 \cite{Goel16SpiroCall} & Sound & & No & No & Limited & Mean error of 4 lung function indices: $ 7.2\% $ \\
\hline

Song, 2020 \cite{Song20Spirosonic} & Acoustic & 0.2m & No & No & Extensive & Healthy human: $\le 3\% $ \\
{} & {} & {} & {} & {}& {} & Pediatric patients: $5\% \sim 10\% $\\
\hline

Massagram, 2009 \cite{Massagram09wifi} & RF & & No & Yes & None & $5 \%$ of the spirometer\\
\hline

Nguyen, 2016 \cite{Nguyen16wifi} & RF & & No & Yes & None &  Median accuracy: $ 90\% \sim 95.4\% $\\
\hline

\textbf{SpiroFi} & \textbf{WiFi} & \textbf{} & \textbf{No} & \textbf{No} & \textbf{Extensive} &  \\
\hline

%\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
% \label{Reftab}
\end{center}
\vspace{-0.03\textheight} % 调整纵向距离

\end{table*}

==> Table/Table2.tex <==
\begin{table}[ht]
\label{tab:Demographics}
\caption{Subject Demographics }
\vspace{-1ex}
% \caption {Comparison of technologies measuring human breathe volume out of clinic}
\begin{center}
\begin{tabular}{|c|c|c|}

\hline
\textbf{Category} & \textbf{Characteristics} & \textbf{Number}\\
\hline
~ & Patient Num. & 34 \\
\cline{2-3}
{Demo-} & Test per person & {7.1$\pm$ 1.6}\\
\cline{2-3}
{graphics} & Validate Test per person & {3.6$\pm$ 1.5}\\
\cline{2-3}
{} & Female($\%$) & 12 (35.2$\%$)\\
\hline
{} & Age (years) & 66.7 $\pm$ 15.6 \\
\cline{2-3}
{Body} & Height(cm) & 166.4 $\pm$ 7.7 \\
\cline{2-3}
{Conditions} & Weight(kg) & 69.1 $\pm$ 16.1\\
\cline{2-3}
{} & BMI(kg/m$^2$) & 24.9 $\pm$ 5.2 \\
\hline
{} & Coronary Heart Disease($\%$) & 64.7 $\%$\\
\cline{2-3}
Diseases & High Blood Pressure ($\%$) & 58.8 $\%$\\
\cline{2-3}
{} & Brain Infarction ($\%$) & 29.4 $\%$ \\
\cline{2-3}
{} & Heart Failure ($\%$) & 17.6 $\%$ \\
\hline

\end{tabular}
\end{center}
\vspace{-0.03\textheight} % 调整纵向距离
\end{table}

==> Table/Table_feature.tex <==
\begin{table}[ht]
\label{tab:feature}
% \vspace{-0.02\textheight} % 调整纵向距离
\caption{Explanation of chest motion features. }
% \vspace{-0.03\textheight} % 调整纵向距离
\begin{center}
\begin{tabular}{|c|c|c|ll}
\cline{1-3}
\multirow{2}{*}{Feature} & \multirow{2}{*}{Physical Meaning} & Corresponding \\
{} & {} & Indice & \\ 
\cline{1-3}
%$S_{max}$ & the maximum speed & $PEF$ &  \\ \cline{1-3}
\multirow{2}{*}{$D_{1s}$}  & the exhalation within & \multirow{2}{*}{$FEV_1$}  \\
{} & {the first second} & {}\\
\cline{1-3}
$D_{max}$ & the maximum displacement  & $FVC$ &  \\ \cline{1-3}
\end{tabular}
\end{center}
\vspace{-0.02\textheight} % 调整纵向距离
\end{table}



==> Table/demographics_lab.tex <==
\begin{table}[ht]
% \vspace{-0.02\textheight}
\caption{Subject Demographics }
\vspace{-0.02\textheight}
% \caption {Comparison of technologies measuring human breathe volume out of clinic}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Category} & \textbf{Characteristics} & \textbf{Number}\\
\hline
{Demo-} & Patient Num. & 10 \\
\cline{2-3}
{graphics} & Test per person & {39.2$\pm$ 4.6}\\
\cline{2-3}
{} & Female($\%$) & 5 (50$\%$)\\
\hline
{} & Age (years) & 22.9 $\pm$ 1.4 \\
\cline{2-3}
{Body} & Height(cm) & 170.1 $\pm$ 7.1 \\
\cline{2-3}
{Conditions} & Weight(kg) & 58.9 $\pm$ 9.1\\
\cline{2-3}
{} & Body Mass Index (BMI) & \multirow{2}{*}{20.3 $\pm$ 2.5} \\
{} &(kg/m$^2$)&{}\\ 
\cline{2-3}
{} & Normal ($\%$) & 8(80$\%$)\\
\cline{2-3}
{} & Underweight ($\%$) & 2 (20$\%$) \\
\cline{2-3}
%{} & Overweight ($\%$) & 1 (10$\%$) \\
\hline

\end{tabular}
\vspace{-0.02\textheight}
\label{tab:demoLab}
\end{center}
\end{table}

==> Table/releTable.tex <==
\begin{table*}[htbp]
\caption{Comparison of technologies measuring human breathe volume out of clinic}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{} & \textbf{Signal} &  \textbf{Physical} & \textbf{Specialized} & \textbf{Clinical} & \textbf{Maneuver errors} & \textbf{Performance}  \\
\textbf{} & \textbf{} &  \textbf{contact} & \textbf{device}  & \textbf{validation} & \textbf{handling} & \textbf{} \\
\hline

Gupta, 2011 \cite{Gupta11sensor} & Sensor & Yes & Yes & Limited & Yes & SD:$\leq 8\%$\\
\hline

Chu, 2019 \cite{Chu19sensor} & Sensor & Yes & Yes & Limited & No & CC: $0.929 \sim 0.962$ \\
\hline

Lewis, 2011 \cite{Lewis11vision} & Vision & No & Yes & None &  No & CC: $0.9$\\
\hline

Yu, 2012 \cite{Yu12vision}  & Vision &Yes & Yes & None & No & CC: $0.966$\\
\hline

Larson, 2012 \cite{Larson12Spirosmart} & Sound & No & No & Limited & No & ME: $ 5.1\% $ \\
\hline

Goel, 2016 \cite{Goel16SpiroCall} & Sound & No & No & Limited & Yes & MSD: $ 7.2\% $ \\
\hline

Song, 2020 \cite{Song20Spirosonic} & Acoustic  & No & No & Extensive & Yes & MSD: $\le 3\% $ \\
\hline

Massagram, 2009 \cite{Massagram09wifi} & RF  & No & Yes & None & No & SD:$5 \%$ \\
\hline

Nguyen, 2016 \cite{Nguyen16wifi} & RF & No & Yes & None & No & ME: $ 4.6\% \sim 10\% $\\
\hline

\multirow{2}{*}{\textbf{SpiroFi}} & \multirow{2}{*}{\textbf{WiFi}} & \multirow{2}{*}{\textbf{No}} & \multirow{2}{*}{\textbf{No}} & \multirow{2}{*}{\textbf{Extensive}} & \multirow{2}{*}{\textbf{Yes}} & \textbf{ME in Lab \& Clinic:}\\

% \textbf{SpiroFi} & \textbf{WiFi}  & \textbf{No} & \textbf{No} & \textbf{Extensive} & \textbf{Yes} & \textbf{ME in Lab \& Clinic:}\\
{} & {} & {} & {} & {} & {} & \textbf{2.55\% \& 6.05\%} \\
\hline
\multicolumn{7}{|c|}{\begin{tabular}[c]{@{}c@{}}\textbf{SD: Standard Deviation; CC: Correlation Coefficient; ME: Mean Error; MSD: Mean Standard Deviation}\end{tabular}}\\
\hline

%\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{Reftab}
\end{center}

\vspace{-0.03\textheight} % 调整纵向距离

\end{table*}

==> Table1.tex <==
\begin{table*}[htbp]
\caption{Comparison of technologies measuring human breathe volume out of clinic}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{} & \textbf{Signal} & \textbf{Sensing} & \textbf{Physical} & \textbf{Specialized} & \textbf{Clinical} & \textbf{Performance}  \\
\textbf{} & \textbf{} & \textbf{range} &  \textbf{contact} & \textbf{device}  & \textbf{validation} & \textbf{} \\
\hline

Gupta, 2011\cite{Gupta11sensor} & Sensor  &  0m & Yes & Yes & Limited & Flow detection rate: $\geq 92\% $ \\
{} & {} & {} & {} & {} & {} & cough detection rate: $\geq 95\% $ \\
\hline

Chu, 2019 \cite{Chu19sensor} & Sensor & 0m & Yes & Yes & Limited & Correlation coefficient: $0.929 \sim 0.962$ \\
\hline

Lewis, 2011 \cite{Lewis11vision} & Vision & & No & Yes & None &  Within-Subject correlation: $0.9$\\
\hline

Yu, 2012 \cite{Yu12vision} & Vision &   & Yes & Yes & None & Correlation coefficient: $r=0.966$\\
\hline

Larson, 2012 \cite{Larson12Spirosmart} & Sound & & No & No & Limited & Compared to a clinical spirometer: $ 5.1\% $ \\
\hline

Goel, 2016 \cite{Goel16SpiroCall} & Sound & & No & No & Limited & Mean error of 4 lung function indices: $ 7.2\% $ \\
\hline

Song, 2020 \cite{Song20Spirosonic} & Acoustic & 0.2m & No & No & Extensive & Healthy human: $\le 3\% $ \\
{} & {} & {} & {} & {}& {} & Pediatric patients: $5\% \sim 10\% $\\
\hline

Massagram, 2009 \cite{Massagram09wifi} & RF & & No & Yes & None & $5 \%$ of the spirometer\\
\hline

Nguyen, 2016 \cite{Nguyen16wifi} & RF & & No & Yes & None &  Median accuracy: $ 90\% \sim 95.4\% $\\
\hline

\textbf{SpiroFi} & \textbf{WiFi} & \textbf{} & \textbf{No} & \textbf{No} & \textbf{Extensive} &  \\
\hline

%\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
% \label{Reftab}
\end{center}
\vspace{-0.03\textheight} % 调整纵向距离

\end{table*}

==> Table2.tex <==
\begin{table}[ht]
\label{tab:Demographics}
\caption{Subject Demographics }
\vspace{-1ex}
% \caption {Comparison of technologies measuring human breathe volume out of clinic}
\begin{center}
\begin{tabular}{|c|c|c|}

\hline
\textbf{Category} & \textbf{Characteristics} & \textbf{Number}\\
\hline
~ & Patient Num. & 34 \\
\cline{2-3}
{Demo-} & Test per person & {7.1$\pm$ 1.6}\\
\cline{2-3}
{graphics} & Validate Test per person & {3.6$\pm$ 1.5}\\
\cline{2-3}
{} & Female($\%$) & 12 (35.2$\%$)\\
\hline
{} & Age (years) & 66.7 $\pm$ 15.6 \\
\cline{2-3}
{Body} & Height(cm) & 166.4 $\pm$ 7.7 \\
\cline{2-3}
{Conditions} & Weight(kg) & 69.1 $\pm$ 16.1\\
\cline{2-3}
{} & BMI(kg/m$^2$) & 24.9 $\pm$ 5.2 \\
\hline
{} & Coronary Heart Disease($\%$) & 64.7 $\%$\\
\cline{2-3}
Diseases & High Blood Pressure ($\%$) & 58.8 $\%$\\
\cline{2-3}
{} & Brain Infarction ($\%$) & 29.4 $\%$ \\
\cline{2-3}
{} & Heart Failure ($\%$) & 17.6 $\%$ \\
\hline

\end{tabular}
\end{center}
\vspace{-0.03\textheight} % 调整纵向距离
\end{table}

==> releTable.tex <==
\begin{table*}[htbp]
\caption{Comparison of technologies measuring human breathe volume out of clinic}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{} & \textbf{Signal} &  \textbf{Physical} & \textbf{Specialized} & \textbf{Clinical} & \textbf{Maneuver errors} & \textbf{Performance}  \\
\textbf{} & \textbf{} &  \textbf{contact} & \textbf{device}  & \textbf{validation} & \textbf{handling} & \textbf{} \\
\hline

Gupta, 2011 \cite{Gupta11sensor} & Sensor & Yes & Yes & Limited & Yes & SD:$\leq 8\%$\\
\hline

Chu, 2019 \cite{Chu19sensor} & Sensor & Yes & Yes & Limited & No & CC: $0.929 \sim 0.962$ \\
\hline

Lewis, 2011 \cite{Lewis11vision} & Vision & No & Yes & None &  No & CC: $0.9$\\
\hline

Yu, 2012 \cite{Yu12vision}  & Vision &Yes & Yes & None & No & CC: $0.966$\\
\hline

Larson, 2012 \cite{Larson12Spirosmart} & Sound & No & No & Limited & No & ME: $ 5.1\% $ \\
\hline

Goel, 2016 \cite{Goel16SpiroCall} & Sound & No & No & Limited & Yes & MSD: $ 7.2\% $ \\
\hline

Song, 2020 \cite{Song20Spirosonic} & Acoustic  & No & No & Extensive & Yes & MSD: $\le 3\% $ \\
\hline

Massagram, 2009 \cite{Massagram09wifi} & RF  & No & Yes & None & No & SD:$5 \%$ \\
\hline

Nguyen, 2016 \cite{Nguyen16wifi} & RF & No & Yes & None & No & ME: $ 4.6\% \sim 10\% $\\
\hline

\multirow{2}{*}{\textbf{SpiroFi}} & \multirow{2}{*}{\textbf{WiFi}} & \multirow{2}{*}{\textbf{No}} & \multirow{2}{*}{\textbf{No}} & \multirow{2}{*}{\textbf{Extensive}} & \multirow{2}{*}{\textbf{Yes}} & \textbf{ME in Lab \& Clinic:}\\

% \textbf{SpiroFi} & \textbf{WiFi}  & \textbf{No} & \textbf{No} & \textbf{Extensive} & \textbf{Yes} & \textbf{ME in Lab \& Clinic:}\\
{} & {} & {} & {} & {} & {} & \textbf{2.55\% \& 6.05\%} \\
\hline
\multicolumn{7}{|c|}{\begin{tabular}[c]{@{}c@{}}\textbf{SD: Standard Deviation; CC: Correlation Coefficient; ME: Mean Error; MSD: Mean Standard Deviation}\end{tabular}}\\
\hline

%\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{Reftab}
\end{center}

\vspace{-0.03\textheight} % 调整纵向距离

\end{table*}
